EM-WaveHoltz: A flexible frequency-domain method built from time-domain solvers

A novel approach to computing time-harmonic solutions of Maxwell's equations by time-domain simulations is presented. The method, EM-WaveHoltz, results in a positive definite system of equations which makes it amenable to iterative solution with the conjugate gradient method or with GMRES. Theoretical results guaranteeing the convergence of the method away from resonances is presented. Numerical examples illustrating the properties of EM-WaveHoltz are given.

==> plan.tex <==
\section{Plan for numerical section}

\begin{itemize}
\item 2D convergence
	\begin{itemize}
	\item standing mode, just sin, cos, $E_z = (x-1)^2x^2(y-1)^2y^2$ for the yee scheme
		\begin{itemize}
		\item grid convergence for the yee scheme
		\item time error elimination
		\end{itemize}
	\end{itemize}
	\item DG + geometry
	\item convergence vs $\omega$ (6 geometries)
	\item The source near the boundary, different recursions in the DAB.
	\item Examples simialr to Bill's 
\item 3D
	\begin{itemize}
	\item Plane and free boundary
	\end{itemize}
\end{itemize}




